Knowledge Distillation as Efficient Pre-training: Faster Convergence, Higher Data-efficiency, and Better Transferability

Large-scale pre-training has been proven to be crucial for various computer vision tasks. However, with the increase of pre-training data amount, model architecture amount, and the private/inaccessible data, it is not very efficient or possible to pre-train all the model architectures on large-scale datasets. In this work, we investigate an alternative strategy for pre-training, namely Knowledge Distillation as Efficient Pre-training (KDEP), aiming to efficiently transfer the learned feature representation from existing pre-trained models to new student models for future downstream tasks. We observe that existing Knowledge Distillation (KD) methods are unsuitable towards pre-training since they normally distill the logits that are going to be discarded when transferred to downstream tasks. To resolve this problem, we propose a feature-based KD method with non-parametric feature dimension aligning. Notably, our method performs comparably with supervised pre-training counterparts in 3 downstream tasks and 9 downstream datasets requiring 10x less data and 5x less pre-training time. Code is available at https://github.com/CVMI-Lab/KDEP.

==> latex_preamble.tex <==
%%%%%%%%  Packages
\usepackage{abstract}
\usepackage{amsfonts,amsmath,amssymb,amsthm}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{dsfont}
% \usepackage{subcaption}
\usepackage{eucal} % nice \mathcal
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{mathtools}
\usepackage{natbib}
\usepackage{soul}
\usepackage{stmaryrd}
\usepackage{thmtools,thm-restate}
\usepackage{tikz}
\usepackage{xcolor}

\usetikzlibrary{positioning}

%%%%%%%%  Toggles
\newif\iffig

%%%%%%%%  Remove abstract title
\renewcommand{\abstractname}{}    
\renewcommand{\absnamepos}{empty}

%%%%%%%%  Paragraph indentation 
\newlength{\zparindent}
\setlength{\zparindent}{\parindent}
\newcommand{\pindent}{\hspace*{\zparindent}}

%%%%%%%%  Typesetting
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\vb}[1]{\texttt{#1}}

\newcommand{\red}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\green}[1]{\textbf{\textcolor{green}{#1}}}
\newcommand{\blue}[1]{\textbf{\textcolor{blue}{#1}}}
\newcommand{\white}[1]{\textbf{\textcolor{white}{#1}}}

%%%%%%%%  Operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\Argmin}{Arg\,min}
\DeclareMathOperator*{\Argmax}{Arg\,max}
\DeclareMathOperator*{\E}{\mathbb E}
\DeclareMathOperator*{\p}{\mathbb P}

%%%%%%%%  Paired operators
\newcommand{\abs}[1]{{\left| #1 \right|}}
\newcommand{\norm}[1]{{\left\| #1 \right\|}}
\newcommand{\nnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\lrangle}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\braces}[1]{{\left\{ #1 \right\}}}
\newcommand{\brackets}[1]{{\left[ #1 \right]}}
\newcommand{\paren}[1]{{\left( #1 \right)}}
\newcommand{\ceil}[1]{{\left\lceil #1 \right\rceil}}

%%%%%%%%  Environments
\declaretheorem{assumption}
\declaretheorem{corollary}
\declaretheorem{definition}
\declaretheorem{example}
\declaretheorem{lemma}
\declaretheorem{observation}
\declaretheorem{property}
\declaretheorem{proposition}
\declaretheorem{remark}
\declaretheorem{reminder}
\declaretheorem{theorem}

\newtheorem{auxlemma}{Lemma}
\newenvironment{lemma*}[1]
  {\renewcommand\theauxlemma{#1}\auxlemma}
  {\endauxlemma}

%%%%%%%%  Symbols
\newcommand{\pd}[2]{{\frac{\partial #1}{\partial #2}}}
\newcommand{\dd}[2]{{\frac{\mathrm{d} #1}{\mathrm{d} #2}}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\C}{^\mathsf{c}}
\newcommand{\T}{^\intercal}

\newcommand{\I}{\mathbb I}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}

% \mathbb
\newcommand{\bA}{\mathbb A}
\newcommand{\bB}{\mathbb B}
\newcommand{\bC}{\mathbb C}
\newcommand{\bD}{\mathbb D}
\newcommand{\bE}{\mathbb E}
\newcommand{\bF}{\mathbb F}
\newcommand{\bG}{\mathbb G}
\newcommand{\bH}{\mathbb H}
\newcommand{\bI}{\mathbb I}
\newcommand{\bJ}{\mathbb J}
\newcommand{\bK}{\mathbb K}
\newcommand{\bL}{\mathbb L}
\newcommand{\bM}{\mathbb M}
\newcommand{\bN}{\mathbb N}
\newcommand{\bO}{\mathbb O}
\newcommand{\bP}{\mathbb P}
\newcommand{\bQ}{\mathbb Q}
\newcommand{\bR}{\mathbb R}
\newcommand{\bS}{\mathbb S}
\newcommand{\bT}{\mathbb T}
\newcommand{\bU}{\mathbb U}
\newcommand{\bV}{\mathbb V}
\newcommand{\bW}{\mathbb W}
\newcommand{\bX}{\mathbb X}
\newcommand{\bY}{\mathbb Y}
\newcommand{\bZ}{\mathbb Z}

% \mathcal
\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

% \mathbf
\newcommand{\f}[1]{\mathbf{#1}}
\newcommand{\fa}{\mathbf a}
\newcommand{\fb}{\mathbf b}
\newcommand{\fc}{\mathbf c}
\newcommand{\fd}{\mathbf d}
\newcommand{\fe}{\mathbf e}
\newcommand{\ff}{\mathbf f}
\newcommand{\fg}{\mathbf g}
\newcommand{\fh}{\mathbf h}
% \newcommand{\fi}{\mathbf i}
\newcommand{\fj}{\mathbf j}
\newcommand{\fk}{\mathbf k}
\newcommand{\fl}{\mathbf l}
\newcommand{\fm}{\mathbf m}
\newcommand{\fn}{\mathbf n}
\newcommand{\fo}{\mathbf o}
\newcommand{\fp}{\mathbf p}
\newcommand{\fq}{\mathbf q}
\newcommand{\fr}{\mathbf r}
\newcommand{\fs}{\mathbf s}
\newcommand{\ft}{\mathbf t}
\newcommand{\fu}{\mathbf u}
\newcommand{\fv}{\mathbf v}
\newcommand{\fw}{\mathbf w}
\newcommand{\fx}{\mathbf x}
\newcommand{\fy}{\mathbf y}
\newcommand{\fz}{\mathbf z}

\newcommand{\fA}{\mathbf A}
\newcommand{\fB}{\mathbf B}
\newcommand{\fC}{\mathbf C}
\newcommand{\fD}{\mathbf D}
\newcommand{\fE}{\mathbf E}
\newcommand{\fF}{\mathbf F}
\newcommand{\fG}{\mathbf G}
\newcommand{\fH}{\mathbf H}
\newcommand{\fI}{\mathbf I}
\newcommand{\fJ}{\mathbf J}
\newcommand{\fK}{\mathbf K}
\newcommand{\fL}{\mathbf L}
\newcommand{\fM}{\mathbf M}
\newcommand{\fN}{\mathbf N}
\newcommand{\fO}{\mathbf O}
\newcommand{\fP}{\mathbf P}
\newcommand{\fQ}{\mathbf Q}
\newcommand{\fR}{\mathbf R}
\newcommand{\fS}{\mathbf S}
\newcommand{\fT}{\mathbf T}
\newcommand{\fU}{\mathbf U}
\newcommand{\fV}{\mathbf V}
\newcommand{\fW}{\mathbf W}
\newcommand{\fX}{\mathbf X}
\newcommand{\fY}{\mathbf Y}
\newcommand{\fZ}{\mathbf Z}
